Generation and De-Identification of Indian Clinical Discharge Summaries using LLMs

The consequences of a healthcare data breach can be devastating for the patients, providers, and payers. The average financial impact of a data breach in recent months has been estimated to be close to USD 10 million. This is especially significant for healthcare organizations in India that are managing rapid digitization while still establishing data governance procedures that align with the letter and spirit of the law. Computer-based systems for de-identification of personal information are vulnerable to data drift, often rendering them ineffective in cross-institution settings. Therefore, a rigorous assessment of existing de-identification against local health datasets is imperative to support the safe adoption of digital health initiatives in India. Using a small set of de-identified patient discharge summaries provided by an Indian healthcare institution, in this paper, we report the nominal performance of de-identification algorithms (based on language models) trained on publicly available non-Indian datasets, pointing towards a lack of cross-institutional generalization. Similarly, experimentation with off-the-shelf de-identification systems reveals potential risks associated with the approach. To overcome data scarcity, we explore generating synthetic clinical reports (using publicly available and Indian summaries) by performing in-context learning over Large Language Models (LLMs). Our experiments demonstrate the use of generated reports as an effective strategy for creating high-performing de-identification systems with good generalization capabilities.

==> sections/acknowledgment.tex <==
\section{Acknowledgment} \label{sec:acknowledgment}

==> sections/summary-generation.tex <==
% \section{Synthetic Discharge Summary Generation for Indian Context} \label{sec:syngen}

% This section presents the approach used to generate synthetic discharge summaries tailored for the Indian context using the one-shot prompting technique in Large Language Models (LLMs) using the n2c2 2006 dataset and \dataReal \ dataset.\ We also discussed the steps involved in filtering generated discharge summaries and the evaluation of quality and annotations of the generated summaries by domain experts and annotators, respectively. 

% \subsection{Discharge Summaries generation using n2c2 2006 dataset}
% We explored synthetic annotated summary generation using Gemini-pro-1.0 using in-context learning approach. We utilize the n2c2 2006 dataset for generating annotated discharge summaries. We gave a specific prompt given in table \ref{tab:prompts-for-ds-gen} to Gemini-pro-1.0 for generating Indian patient discharge summary.\ We come up with this prompt after extensive prompt tuning. We generated five Indian patient discharge summaries from one prompt + n2c2 2006 discharge summary. In total, we generated 3000 discharge summaries. After generating the summaries, we manually filtered them using the rules mentioned in section 4.3. After filtering, we have 1603 annotated summaries and named them {\dataGenGemini}.

% We analyzed the {\ncOld} and the synthetic {\dataGenGemini} discharge summaries in terms of summary statistics, Jaccard distance, and BERTScore (using the "dmis-lab/biobert-v1.1" model) as shown in \ref{tab:datasetn2c2} (\cite{lee2020biobert}). The Jaccard distance measures the dissimilarity between two sets, where a value closer to 1 indicates greater dissimilarity. BERTScore, on the other hand, leverages the BERT language model embeddings to compute the cosine similarity between the tokens of two texts \cite{zhang2020bertscore}. BERTScore provides three key measures: precision (how much each token in the candidate text is semantically similar to any token in the reference text), recall (how well each token in the reference text is semantically captured by the candidate text), and F1 score (the harmonic mean of precision and recall). The Jaccard distance suggests a high level of dissimilarity between the datasets, indicating that the synthetic dataset introduces a significant degree of variation compared to the real dataset. The F1 score of 0.6362, while indicating some differences, also suggests a reasonable level of overlap in the semantic content between the datasets. Precision slightly exceeds recall, indicating that while the synthetic texts are fairly representative of the real texts, they occasionally introduce content not present in the real dataset. This is aligned with the goal of generating synthetic data that, while similar to the real dataset, introduces new elements to enhance robustness or coverage in modeling tasks. An n-gram analysis of the top 10 unigrams, bigrams, and trigrams unveils the differences between the two datasets, yet also underscores their relevance to the task at hand as shown in Figure~\ref{fig:n2c2realngrams}, Figure~\ref{fig:n2c2synngrams}, Figure~\ref{fig:PHIn2c2ngrams}, and Figure~\ref{fig:PHIn2c2synngrams}. 

% These metrics suggest that while the synthetic dataset is designed to be distinct enough to introduce useful variability, it retains a substantive semantic similarity to the real dataset. This balance is crucial when synthetic data is used for tasks such as model training, where the goal is to ensure that the model is not only trained on a diverse set of data but also remains relevant and effective when applied to real-world data. The high Jaccard distance combined with the moderate BERTScore indicates that the synthetic dataset achieves this objective by being similar enough to the real dataset to be useful, yet different enough to enhance the dataset's diversity and robustness.

% \begin{table}[b] 
% \centering
% \scalebox{0.63}{
% \begin{tabular}{@{}lcc@{}}
% \toprule
% Attribute & \multicolumn{2}{c}{Dataset} \\ \cmidrule(l){2-3} 
%  & Real & Synthetic \\ \midrule
% Counts & 3158684 & 5022667 \\
% Length (words) & 560753 & 721886 \\
% Mean $\pm$ SE & 4.63293 $\pm$ 0.00428 (62) & 5.93219 $\pm$ 0.00565 (9465) \\
% Median & 4.0 & 5.0 \\
% Min & 1 & 1 \\
% Max & 50 & 89 \\
% Jaccard Distance & \centering 0.8251 & \centering \\
% BERTScore (F1) & \centering 0.6362 & \centering \\
% BERTScore (Precision) & \centering 0.6451 & \centering \\
% BERTScore (Recall) & \centering 0.6276 & \centering \\ \bottomrule
% \end{tabular}}
% \caption{Comparison of n2c2 2006 and {\dataGenGemini} Dataset}
% \label{tab:datasetn2c2}
% \end{table}

% \subsection{Discharge Summaries generation using \dataReal \ dataset}
% We explored synthetic annotated summary generation using \dataReal\ dataset through experimentation with multiple open-source in-premise setup LLMs and different prompts.\ Specifically, we tested with three distinct LLMs and two different prompts (i.e.\ Table \ref{tab:prompts-for-ds-gen}), resulting in a total of five model-prompt combinations.\ Our objective was to identify the most effective model-prompt combination which generates summaries which closely resemble the discharge summaries in  \dataReal\ dataset.

% To evaluate the performance of model-prompt combinations, we calculated metrics such as BERT F1-Score and average length of summaries (in words).\ The BERT F1-Score was calculated by comparing 30 synthetic annotated discharge summaries (generated from 5 \dataReal\ discharge summaries) and 99 original \dataReal\ discharge summaries.\ The average summary length (in words) is calculated using 30 synthetic annotated discharge summaries.\ The results of these experiments are mentioned in Table \ref{tab:model-prompt-comparison}.\ The BERT F1-Score of Meta-Llama-3-8B-Instruct and Mistral-7B-Instruct-v0.1 models with prompt A surpasses that of other model-prompt combinations, indicating a significant similarity in their performance.\ We selected Meta-Llama-3-8B-Instruct model for synthetic annotated discharge summary generation as the BERT F1-score is high and average length of annotated generated summaries is highest among other model-prompt combinations.\ 

% For generating diverse synthetic annotated discharge summaries, temperature of the model i.e.\ Meta-Llama-3-8B-Instruct was set to 0.9 and around 25 summaries were generated from each of the \dataReal\ discharge summaries numbered 01 to 79, where synthetic summaries generated from 01 to 79 \dataReal\ summaries after filtering were used in the training set.\ The \dataReal\ discharge summaries numbered 80 to 99 were not used to generate synthetic summaries, as these \dataReal\ summaries were used in the testing set.

% Similar to the n2c2 datasets, we analyzed the \dataReal\ and \dataGenLlama datasets with summary statistics, Jaccard distance, and BERTScore, as shown in Table 2. The Jaccard distance for this pair shows a substantial level of dissimilarity. This indicates a significant introduction of new elements in the synthetic dataset.The BERTScore results indicate a moderate level of semantic similarity between the real and synthetic datasets. The precision is higher than the recall, suggesting that the synthetic dataset generally includes content that is semantically relevant to the real dataset but may not capture all the semantic nuances of the real data.These metrics indicate that this synthetic dataset introduces a higher level of variation. The Jaccard distance and BERTScore together suggest that the synthetic dataset effectively diversifies the data landscape. Furthermore, an n-gram analysis of the top 10 unigrams, bigrams, and trigrams reveals the differences the distinct yet semantically relevant nature of the two datasets as shown in Figure~\ref{fig:sgpgirealngrams}, Figure~\ref{fig:sgpgisynngrams}, Figure~\ref{fig:PHIsgpgirealngrams}, and Figure~\ref{fig:PHIsgpgisynngrams}. 

% \begin{table}[ht]
% \centering
% \scalebox{0.725}{
% \begin{tabular}{@{}lcc@{}}
% \toprule
% Attribute & \multicolumn{2}{c}{Dataset} \\ \cmidrule(l){2-3} 
%  & Real & Synthetic \\ \midrule
% Counts & 636805 & 4789863 \\
% Length (words) & 102604 & 508244 \\
% Mean $\pm$ SE & 5.20644 $\pm$ 0.01039 & 7.76700 $\pm$ 0.01081 \\
% Median & 4.0 & 5.0 \\
% Min & 1 & 1 \\
% Max & 72 & 472 \\
% Jaccard Distance & \centering 0.8022 & \centering \\
% BERTScore (F1) & \centering 0.5780 & \centering \\
% BERTScore (Precision) & \centering 0.5975 & \centering \\
% BERTScore (Recall) & \centering 0.5596 & \centering \\ \bottomrule
% \end{tabular}}
% \caption{Comparison of \dataReal and \dataGenLlama \ Dataset}
% \label{tab:dataset_ICSD-R}
% \end{table}


% \begin{table*}[t]
%     \centering
%     \scalebox{0.76}{
%     \begin{tabular}{cccc}
%         \hline

%         \textbf{Prompt Id} & \textbf{Model Used} & \textbf{BERT F1-Score} & \textbf{Average summary} \\
%           &  &  & \textbf{length (in words)} \\
%         \hline
%         A & meta-llama/Meta-Llama-3-8B-Instruct  & 0.491 & 564\\

%         A & mistralai/Mistral-7B-Instruct-v0.1 & 0.493 & 400 \\
   
%                 B & meta-llama/Meta-Llama-3-8B-Instruct & 0.486 &503\\
    
%         B & mistralai/Mistral-7B-Instruct-v0.1 & 0.468 & 267\\
       
%                 B & google/gemma-1.1-7b-it & 0.478 &268 \\
%         \hline
%   \end{tabular}}
%     \caption{Comparison of model-prompt combinations}
%     \label{tab:model-prompt-comparison}
% \end{table*}

% \subsection{Filtering of generated summaries}
% We generated around 3000 synthetic discharge summaries from n2c2 2006 dataset using gemini and around 1831 synthetic discharge summaries from \data\ dataset using Meta-Llama-3-8B-Instruct model.\ These generated discharge summaries were manually filtered to discard the summaries that contain gibberish, include annotations for entities not specified in the prompt, incorrect annotations or unannotated summaries.\ After manual filtering, we got around 1596 annotated summaries from n2c2 2006 dataset and named it ICDS-G(g) dataset and around 1043 annotated summaries from \data\ dataset and named it ICDS-G(l) dataset.\ These annotated summaries were subsequently used for further experiments.
 


% \subsection{Evaluation of Quality of Generated Summaries by Domain Experts}
% We assessed the face validity of the generated summaries by asking physicians to review a convenience sample of 30 real and 30 synthetic discharge summaries with the real/synthetic labels surpassed. The 60 discharge summaries were shuffled and uploaded to a secure, online review tool accessible only to the reviewers. The reviewers were asked to review each summary and then assign a single label (real or synthetic) to each based on their experience. The results of the review were compiled and the precision, recall and F1 scores were computed for each physician along with Cohen's Kappa to assess agreement between the two physicians.

% The confusion matrix on convenience sample of 60 discharge summaries evaluated by physician1 and physician2 are shown in Figure \ref{fig:cm_physician1} and Figure \ref{fig:cm_physician2} respectively.\ There are 10 summaries which were originally synthetic but were labeled as real by physician 1 and 19 summaries which were originally synthetic but were labeled as real by physician 2.\ Physician 1 is able to label summaries with higher precision and recall i.e. higher f1-score as compared to physician 2 (Table \ref{tab:em_physician1_physician2}).\ The Cohen's kappa coefficient i.e.\ the measure of inter-annotator agreement is 0.290 which shows a fair agreement between assigned labels by the physicians. 
%  % We can observe that physician 1 is able to label almost 75\% of summaries correctly where as physician 2 is able to label almost 55\% of summaries correctly.
 
% Additionally the physician\ 1\ observed that among the discharge summaries that he labeled synthetic, many appeared to have been translated from a non-English source. Physician 2 reported some issues in diagnosis as well as formatting issues among the summaries he labeled as synthetic. Additionally physician\ 2\ reported some errors in diagnoses, medications and lab results but these were not limited to the summaries that he labeled as synthetic.


% % We randomly sampled fifteen discharge summaries from each n2c2 2006, ICDS-R, ICDS-G(g), and ICDS-G(l) datasets. We have sixty summaries, of which thirty were real and thirty were synthetic. We gave these sampled summaries to medical experts and asked them to classify whether the summaries are synthetic or real. Our Finding is mentioned in table [].




% \subsection{Evaluation of Annotation of Synthetic Summaries by Annotators}
% We randomly sampled fifty summaries from the ICSD-G(l) dataset denote them, and gave these summaries to the annotators to annotate the Summaries with PII tags. We have already annotated summaries with LLM and now with the human annotators, and then we calculated the annotation quality of LLM by comparing these summaries.
